Meta$^2$: Precomputing Reusable Knowledge for Online Harness Evolution in Long-Horizon Agents

Harness optimization improves long-horizon agents by refining the prompts, tools, memory, and hooks around a frozen model. Offline methods can learn from completed trajectories, but deploy one shared harness that may overfit training tasks and cannot react to evidence revealed during a new run. Online evolution can adapt before, during, or after one run through an evolver, but may have to reason about every intervention from scratch or rely on verifier feedback that is usually unavailable at test time. We introduce Meta$^2$, which moves offline optimization one level up: rather than optimizing a shared harness, it learns reusable knowledge for harness evolution and applies it within each task online. Offline, Meta$^2$ learns a textual Meta-Skill $M$ by contrasting training rollouts of the same task agent under three configurations: without an evolver, with an evolver guided by the current version of $M$, and with an evolver given privileged verifier information available only in training. Contrasts in trajectories and outcomes are aggregated across tasks to refine $M$ into reusable guidance on when and how to evolve, when to leave the harness unchanged, and which interventions to avoid. Online, an evolver combines the frozen $M$ with emerging trajectory evidence to decide whether to KEEP the harness unchanged or EVOLVE it through a task-local edit. Each edit applies to the rest of the same run without resetting its environment or progress. Thus, evolution guidance transfers across tasks while harness edits remain task-local, and held-out verifier feedback is never available to the evolver. On two long-horizon benchmarks, Terminal-Bench 2.1 and DeepSWE 1.1, Meta$^2$ achieves the highest performance among evaluated methods with GPT-5.6-Terra, reaching 81.00% and 44.44%, respectively. Ablations support the value of contrastive evolution guidance and keeping online harness edits task-local.

==> assets/diagram-style.tex <==
% Load after TikZ. Mark an explicit right-angle turn with \apbend{coordinate};
% use \apbend[APAccent]{coordinate} to match a differently colored connector.
% Square connector markers are part of both paper and cover layouts.
% Mark an arrow's starting border with \apstart{node.east} or {node.south}.
\providecommand{\apbend}[2][APDark]{%
  \path[fill=#1,draw=none]
    ([xshift=-1.5pt,yshift=-1.5pt]#2) rectangle
    ([xshift=1.5pt,yshift=1.5pt]#2);
}
\providecommand{\apstart}[2][APDark]{\apbend[#1]{#2}}


==> figures/f1_overview.tex <==
% Wide overview: a coordinated team above an uninterrupted deployment timeline.
\begin{figure}[t]
    \centering
    \begingroup
    \definecolor{rhInk}{HTML}{283B50}
    \definecolor{rhBlue}{HTML}{376FA6}
    \definecolor{rhBluePale}{HTML}{EFF5FC}
    \definecolor{rhOrange}{HTML}{B65B27}
    \definecolor{rhOrangePale}{HTML}{FFF3EB}
    \definecolor{rhTeal}{HTML}{287F83}
    \definecolor{rhTealPale}{HTML}{EAF6F4}
    \input{figures/rehearse_icons}
    \begin{tikzpicture}[
        x=.91cm,y=.90cm,
        font=\sffamily\fontsize{8}{9.5}\selectfont,text=rhInk,
        icon/.style={draw=rhInk,line width=.75pt,line cap=round,line join=round},
        flow/.style={-{Stealth[length=4pt,width=3.5pt]},draw=rhInk!75,
                     line width=.7pt,rounded corners=3pt},
        knowledge/.style={flow,draw=rhTeal,line width=1pt},
        guide/.style={flow,dashed,draw=rhBlue!65},
        smallnote/.style={font=\sffamily\fontsize{7}{8.5}\selectfont,align=center},
        heading/.style={font=\sffamily\bfseries\fontsize{10}{12}\selectfont},
        label/.style={font=\sffamily\bfseries\fontsize{8}{9.5}\selectfont},
        card/.style={draw=rhBlue!30,fill=white,rounded corners=4pt,line width=.6pt}
    ]
    \fill[rounded corners=6pt,rhBluePale] (0,-.12) rectangle (7.98,7.17);
    \fill[rounded corners=6pt,rhOrangePale] (8.28,-.12) rectangle (15.2,7.17);
    % Lift the team row to reserve a clear lane for checkpoint labels.
    \begin{scope}[shift={(0,.55)}]
    \node[heading,text=rhBlue] at (3.99,6.20) {Rehearse offline.};
    \node[smallnote] at (3.99,5.80) {Precompute modification experience};
    \node[heading,text=rhOrange] at (11.74,6.20) {Evolve online.};
    \node[smallnote] at (11.74,5.80) {Reuse experience as the task unfolds};

    % One enclosure, spanning both phases, identifies the coordinated team.
    \draw[draw=rhInk!45,fill=white,rounded corners=5pt,line width=.7pt]
      (.22,3.32) rectangle (14.98,5.42);
    \node[label,fill=white,inner sep=3pt] at (7.60,5.42)
      {H-Evolve: coordinated agent team};
    \pic[scale=.66] at (1.43,4.65) {rh-distill};
    \pic[scale=.66] at (4.02,4.65) {rh-summarize};
    \pic[scale=.65] at (6.74,4.65) {rh-database};
    \pic[scale=.66] at (11.63,4.65) {rh-supervisor};
    \node[label] at (1.43,3.98) {Distiller};
    \node[label] at (4.02,3.98) {Summarizer};
    \node[label,text=rhTeal] at (6.74,3.98) {Meta-Skill};
    \node[label] at (11.63,3.98) {Supervisor};
    \node[smallnote,text=rhTeal] at (6.74,3.63) {reusable artifact};
    \node[smallnote] (supervisordecision) at (11.63,3.63) {Keep or Modify};
    \draw[flow] (1.97,4.65) -- (3.48,4.65);
    \node[smallnote,text=rhBlue] at (2.72,4.91) {lessons};
    \draw[flow] (4.55,4.65) -- (6.22,4.65);
    \draw[knowledge] (7.25,4.65) -- (10.94,4.65);
    \node[smallnote,text=rhTeal] at (9.06,4.92) {reuse across tasks};
    \end{scope}

    % Offline inputs stay below the team; the paired evidence feeds distillation.
    \draw[card] (.35,1.40) rectangle (3.79,2.93);
    \node[label] at (2.07,2.67) {Paired training runs};
    \pic[scale=.48] at (1.21,2.13) {rh-document};
    \pic[scale=.48] at (2.93,2.13) {rh-document};
    \node[smallnote] at (1.21,1.66) {worker only};
    \node[smallnote] at (2.93,1.66) {supervised};
    \draw[flow] (1.63,2.13) -- (2.51,2.13);
    \draw[flow] (1.43,2.93) -- (1.43,3.84);
    \draw[card] (4.15,1.40) rectangle (7.63,2.93);
    \node[label] at (5.89,2.67) {Shared guidance};
    \pic[scale=.49] at (5.03,2.13) {rh-profile};
    \pic[scale=.49] at (6.75,2.13) {rh-rubric};
    \node[smallnote] at (5.03,1.66) {error profile};
    \node[smallnote] at (6.75,1.66) {rubric};
    \draw[guide] (5.89,2.93) -- (5.89,3.40) -- (4.02,3.40) -- (4.02,3.84);
    \draw[guide] (4.02,3.40) -- (1.85,3.40) -- (1.85,3.84);
    \node[smallnote] at (3.99,.91) {Training hindsight, not held-out answers};
    \node[smallnote,text=rhBlue] at (3.99,.41)
      {Experience construction: Figure~\ref{fig:experience-construction}};

    % Repeated checkpoints reveal selective evolution, not a single setup edit.
    \node[smallnote,anchor=north,inner sep=1pt] at (8.81,3.43) {Start};
    \node[smallnote,anchor=north,inner sep=1pt]
      (keepdecision) at (10.65,3.43) {Keep};
    \node[smallnote,anchor=north,inner sep=1pt,text=rhOrange]
      (editdecision) at (12.49,3.43) {Modify\\edit};
    \node[smallnote,anchor=north,inner sep=1pt,text=rhOrange]
      (steerdecision) at (14.33,3.43) {Modify\\steer};
    % A shared connector has no arrowheads; straight drops end above labels.
    \draw[draw=rhOrange,line width=.7pt]
      (supervisordecision.south) -- (11.63,3.78)
      (10.65,3.78) -- (14.33,3.78);
    \foreach \x/\decision in {10.65/keepdecision,12.49/editdecision,14.33/steerdecision} {
      \draw[draw=rhOrange,line width=.7pt,
            -{Stealth[length=3pt,width=3pt]},shorten >=2pt]
        (\x,3.78) -- (\decision.north);
    }
    \foreach \x in {8.81,10.65,12.49,14.33} {
      \draw[card,draw=rhOrange!40] (\x-.65,2.05) rectangle (\x+.65,2.76);
      % Draw each component once; a message replaces the context glyph.
      \ifdim\x pt>14pt
        \pic[scale=.30] at (\x-.27,2.51) {rh-speech};
      \else
        \pic[scale=.22] at (\x-.27,2.51) {rh-document};
      \fi
      \ifdim\x pt>12pt
        \fill[rounded corners=1pt,rhOrange!25] (\x+.10,2.35) rectangle (\x+.46,2.67);
        \pic[scale=.28] at (\x+.28,2.51) {rh-settings};
      \else
        \pic[scale=.22] at (\x+.28,2.51) {rh-settings};
      \fi
      \pic[scale=.20] at (\x-.27,2.19) {rh-database};
      \pic[scale=.25] at (\x+.28,2.19) {rh-workflow};
    }
    \node[smallnote] at (8.81,1.85) {$h_0$};
    \node[smallnote] at (10.65,1.85) {$h_0$};
    \node[smallnote,text=rhOrange] at (12.49,1.85) {$h_1$};
    \node[smallnote,text=rhOrange] at (14.33,1.85) {$h_1$ + msg.};
    \draw[flow] (8.44,1.48) -- (15.03,1.48);
    \foreach \x/\t in {8.81/0,10.65/1,12.49/2,14.33/3} {
      \fill[rhInk] (\x,1.48) circle (.045);
      \node[smallnote] at (\x,1.21) {$t_{\t}$};
    }
    \pic[scale=.45] at (8.98,.66) {rh-agent};
    \pic[scale=.45] at (14.53,.66) {rh-terminal};
    % Separate arrow lanes leave room for the label without masking either line.
    \draw[flow,draw=rhBlue] (9.50,.94) -- (13.99,.94);
    \draw[flow,draw=rhOrange] (13.99,.42) -- (9.50,.42);
    \node[smallnote,inner sep=0pt] at (11.74,.68)
      {H-Task $\leftrightarrow$ environment};
    \node[smallnote] at (11.74,.17) {Same task; accumulating feedback; no restart};
    \draw[flow,draw=rhBlue] (14.82,.66) -- (15.11,.66)
      -- (15.11,5.20) -- (12.35,5.20);
    \node[smallnote,text=rhBlue] at (13.75,5.46) {new feedback};
    \end{tikzpicture}
    \endgroup
    \caption{\textbf{\method: a coordinated team for evolution over time.}
    H-Evolve combines an offline distiller (funnel), summarizer (merging lessons),
    and online supervisor. Their handoff is the reusable Meta-Skill. During one
    uninterrupted deployment, keeping leaves the persistent harness at $h_0$;
    an edit produces $h_1$, whose highlighted tool change is retained while a
    later steering message enters context. Each miniature harness shows context,
    tools, memory, and workflow. This illustrative sequence shows modification
    forms and lifetimes, not a required schedule or a measured trajectory.}
    \label{fig:rehearse-overview}
\end{figure}

==> figures/f1_teaser.tex <==
\begin{figure}[t]
    \centering
    \begingroup
    \definecolor{teaserInk}{HTML}{283B50}
    \definecolor{teaserTeal}{HTML}{287F83}
    \definecolor{teaserTealPale}{HTML}{EFF8F7}
    \definecolor{teaserOrange}{HTML}{B65B27}
    \definecolor{teaserOrangePale}{HTML}{FFF4EC}
    \definecolor{teaserBluePale}{HTML}{EFF5FC}
    \definecolor{teaserGrayPale}{HTML}{F3F5F7}
    \resizebox{0.98\linewidth}{!}{%
    \begin{tikzpicture}[
        x=1cm,y=1cm,
        font=\sffamily\fontsize{7.4}{8.8}\selectfont,
        text=teaserInk,
        panel/.style={draw=teaserInk!25,rounded corners=3pt,line width=.65pt},
        box/.style={draw=teaserInk!35,fill=white,rounded corners=2pt,
                   line width=.6pt,align=center,minimum height=.85cm,
                   inner xsep=5pt,inner ysep=3pt},
        arrow/.style={-{Stealth[length=4.5pt,width=4pt]},line width=.9pt,
                      line cap=round},
        header/.style={font=\sffamily\bfseries\fontsize{8.3}{9.7}\selectfont},
        note/.style={font=\sffamily\fontsize{6.7}{7.9}\selectfont,
                     text=teaserInk!78,align=center}
    ]
        \draw[panel,fill=teaserGrayPale] (0,3.55) rectangle (7.85,6.15);
        \node[header,anchor=west] at (.35,5.78)
          {Pre-deployment evolution};
        \node[note,anchor=east] at (7.5,5.78)
          {reusable, but fixed during a run};
        \node[box,text width=1.55cm] (train) at (1.35,4.72)
          {Training\\trajectories\\and outcomes};
        \node[box,text width=1.55cm] (shared) at (4.05,4.72)
          {One shared\\harness\\$h^\star$};
        \node[box,text width=1.55cm] (targets) at (6.65,4.72)
          {All held-out\\tasks};
        \draw[arrow,draw=teaserInk!65] (train) -- (shared);
        \draw[arrow,draw=teaserInk!65] (shared) -- (targets);
        \node[note] at (4.02,3.76)
          {Cannot react to evidence revealed after execution begins};

        \draw[panel,fill=teaserOrangePale] (8.15,3.55) rectangle (16,6.15);
        \node[header,anchor=west,text=teaserOrange] at (8.5,5.78)
          {Within-run evolution};
        \node[note,anchor=east] at (15.65,5.78)
          {reactive, but must reason anew};
        \node[box,text width=1.55cm] (evidence) at (9.5,4.72)
          {Active-run\\evidence\\$\mathcal{I}^{(k)}$};
        \node[box,text width=1.65cm] (scratch) at (12.15,4.72)
          {Choose an edit\\without reusable\\guidance};
        \node[box,text width=1.55cm] (local) at (14.8,4.72)
          {Task-local\\$\delta^{(k)}$};
        \draw[arrow,draw=teaserOrange] (evidence) -- (scratch);
        \draw[arrow,draw=teaserOrange] (scratch) -- (local);
        \node[note] at (12.08,3.76)
          {Repeats intervention reasoning at each checkpoint};

        \draw[panel,fill=teaserBluePale] (0,0) rectangle (16,3.2);
        \node[header,anchor=west] at (.35,2.83)
          {\method: precompute reusable knowledge, then adapt locally};
        \draw[teaserInk!25,dashed,line width=.55pt] (9.55,.38) -- (9.55,2.58);
        \node[header,text=teaserTeal] at (4.65,2.42) {Offline};
        \node[header,text=teaserOrange] at (12.75,2.42) {Within-run};

        \node[box,draw=teaserTeal!55,text width=1.65cm] (contrasts) at (1.6,1.35)
          {A/B/C rollout\\contrasts};
        \node[box,draw=teaserTeal!55,text width=1.8cm] (raa) at (4.65,1.35)
          {\textsc{Reflect}\\\textsc{Aggregate}\\\textsc{Update}};
        \node[box,draw=teaserTeal!65,fill=teaserTealPale,text width=1.55cm]
          (meta) at (7.75,1.35)
          {Frozen\\Meta-Skill\\$\mathcal{M}$};
        \draw[arrow,draw=teaserTeal] (contrasts) -- (raa);
        \draw[arrow,draw=teaserTeal] (raa) -- (meta);

        \node[box,draw=teaserOrange!55,text width=1.65cm] (checkpoint) at (11.05,1.35)
          {$\mathcal{M}+\mathcal{I}^{(k)}$\\at checkpoint $k$};
        \node[box,draw=teaserOrange!65,fill=teaserOrangePale,text width=2.15cm]
          (decision) at (14.25,1.35)
          {\textsc{Keep} or\\\textsc{Evolve}$\bigl(\delta^{(k)}\bigr)$};
        \draw[arrow,draw=teaserTeal] (meta) -- (checkpoint);
        \node[note,text=teaserTeal] at (9.4,1.67) {reused};
        \draw[arrow,draw=teaserOrange] (checkpoint) -- (decision);
        \node[note] at (12.75,.35)
          {Reusable $\mathcal{M}$; task-local $\delta^{(k)}$};
    \end{tikzpicture}%
    }
    \endgroup
    \caption{\textbf{Overview of \method.}
    Pre-deployment evolution reuses one fixed harness, whereas within-run
    evolution can react to active evidence but may lack reusable guidance.
    \method combines the two regimes: it learns a frozen Meta-Skill
    $\mathcal{M}$ from training contrasts and uses it at checkpoints to choose
    \textsc{Keep} or a task-local \textsc{Evolve} edit without restarting the
    task or observing the held-out verifier outcome.}
    \label{fig:teaser-figure}
\end{figure}

==> figures/f2_experience.tex <==
% Icon-led implementation overview of offline learning and online execution.
\begin{figure}[t]
    \centering
    \begingroup
    \definecolor{fInk}{HTML}{17284A}
    \definecolor{fBlue}{HTML}{1764D9}
    \definecolor{fBluePale}{HTML}{F1F7FF}
    \definecolor{fPurple}{HTML}{6B35D5}
    \definecolor{fPurplePale}{HTML}{F7F3FF}
    \definecolor{fTeal}{HTML}{19847D}
    \definecolor{fTealPale}{HTML}{EDF9F7}
    \definecolor{fOrange}{HTML}{C56524}
    \definecolor{fOrangePale}{HTML}{FFF4EA}
    \definecolor{fGray}{HTML}{66758A}
    \definecolor{fGrayPale}{HTML}{F1F3F6}
    \colorlet{rhInk}{fInk}
    \colorlet{rhBlue}{fBlue}
    \colorlet{rhBluePale}{fBluePale}
    \colorlet{rhOrange}{fOrange}
    \colorlet{rhOrangePale}{fOrangePale}
    \colorlet{rhTeal}{fTeal}
    \colorlet{rhTealPale}{fTealPale}
    \resizebox{\textwidth}{!}{%
    \begin{tikzpicture}[
        x=.855cm,y=.80cm,
        font=\sffamily\fontsize{7.1}{8.4}\selectfont,
        text=fInk,
        icon/.style={draw=fInk,line width=.75pt,line cap=round,line join=round},
        flow/.style={-{Stealth[length=4pt,width=3.5pt]},draw=fInk!68,
                     line width=.72pt,rounded corners=3pt},
        deploy/.style={-{Stealth[length=5pt,width=4pt]},draw=fPurple,
                       line width=1.05pt,rounded corners=3pt},
        interaction/.style={-{Stealth[length=4pt,width=3.5pt]},draw=fBlue,
                            dashed,line width=.72pt,rounded corners=3pt},
        offlinecard/.style={draw=fPurple!45,fill=white,rounded corners=4pt,
                            line width=.65pt,align=center},
        onlinecard/.style={draw=fBlue!50,fill=white,rounded corners=4pt,
                           line width=.65pt,align=center},
        heading/.style={font=\sffamily\bfseries\fontsize{9.3}{11}\selectfont},
        title/.style={font=\sffamily\bfseries\fontsize{7.5}{8.8}\selectfont,
                      align=center},
        small/.style={font=\sffamily\fontsize{6.3}{7.5}\selectfont,align=center},
        tiny/.style={font=\sffamily\fontsize{5.8}{6.9}\selectfont,align=center},
        badge/.style={rounded corners=2pt,inner xsep=3pt,inner ysep=1.2pt,
                      font=\sffamily\bfseries\fontsize{5.8}{6.8}\selectfont}
    ]
    \input{figures/rehearse_icons}

    \node[heading] at (7.675,10.05)
      {Meta-Skill-guided online harness evolution};

    % ==================================================================
    % Offline
    % ==================================================================
    \fill[draw=fPurple!35,fill=fPurplePale,rounded corners=7pt,line width=.75pt]
      (0,1.45) rectangle (7.00,9.58);
    \node[heading,anchor=west,text=fPurple] at (.30,9.22)
      {OFFLINE: learn the Meta-Skill};

    % 1. A/B/C rollout collection.
    \draw[offlinecard] (.35,7.45) rectangle (6.65,8.88);
    \node[title,anchor=west] at (.58,8.60) {1. Roll out each training task};
    \node[badge,fill=fPurple!14,text=fPurple] at (6.10,8.60) {LLM};

    \pic[scale=.58] at (1.25,8.03) {rh-agent};
    \node[small] at (1.25,7.62) {A: Agent};

    \pic[scale=.58] at (3.48,8.03) {rh-agent};
    \pic[scale=.30] at (4.02,8.05) {rh-database};
    \node[small] at (3.63,7.62) {B: Evolver + $\mathcal{M}$};

    \pic[scale=.58] at (5.70,8.03) {rh-agent};
    \pic[scale=.34] at (6.22,8.05) {rh-rubric};
    \node[small] at (5.82,7.62) {C: Evolver + verifier};

    \draw[flow,draw=fPurple!70] (3.50,7.45) -- (3.50,7.17);

    % 2. Outcome-conditioned pairing, shown with pass/fail icons.
    \draw[offlinecard,draw=fBlue!42] (.35,5.62) rectangle (6.65,7.17);
    \node[title,anchor=west] at (.58,6.91) {2. Pair terminal outcomes};
    \node[badge,fill=fBlue!12,text=fBlue] at (5.97,6.91) {MECHANICAL};

    \node[badge,fill=fTeal!14,text=fTeal] at (1.30,6.53) {\texttt{act}};
    \node[tiny] at (.72,6.20) {A}; \pic at (1.00,6.20) {rh-fail};
    \draw[flow] (1.18,6.20) -- (1.46,6.20);
    \node[tiny] at (1.66,6.20) {B}; \pic at (1.94,6.20) {rh-pass};
    \node[tiny] at (.72,5.87) {B}; \pic at (1.00,5.87) {rh-fail};
    \draw[flow] (1.18,5.87) -- (1.46,5.87);
    \node[tiny] at (1.66,5.87) {C}; \pic at (1.94,5.87) {rh-pass};

    \node[badge,fill=fOrange!14,text=fOrange] at (3.48,6.53) {\texttt{avoid}};
    \node[tiny] at (2.90,6.20) {A}; \pic at (3.18,6.20) {rh-pass};
    \draw[flow] (3.36,6.20) -- (3.64,6.20);
    \node[tiny] at (3.84,6.20) {B}; \pic at (4.12,6.20) {rh-fail};
    \node[tiny] at (2.90,5.87) {B}; \pic at (3.18,5.87) {rh-pass};
    \draw[flow] (3.36,5.87) -- (3.64,5.87);
    \node[tiny] at (3.84,5.87) {C}; \pic at (4.12,5.87) {rh-fail};

    \node[badge,fill=fBlue!12,text=fBlue] at (5.68,6.53) {\texttt{hold}};
    \node[tiny] at (5.10,6.03) {A}; \pic at (5.38,6.03) {rh-pass};
    \node[small] at (5.72,6.03) {$+$};
    \node[tiny] at (5.96,6.03) {B}; \pic at (6.24,6.03) {rh-pass};

    \draw[flow,draw=fPurple!70] (3.50,5.62) -- (3.50,5.34);

    % 3--5. Icon-led LLM pipeline.
    \draw[offlinecard] (.35,3.42) rectangle (2.25,5.34);
    \node[badge,fill=fPurple!14,text=fPurple] at (1.88,5.08) {LLM};
    \pic[scale=.78] at (1.30,4.55) {rh-distill};
    \node[title] at (1.30,3.88) {3. Write};
    \node[tiny] at (1.30,3.61) {lesson entry};

    \draw[offlinecard] (2.55,3.42) rectangle (4.45,5.34);
    \node[badge,fill=fPurple!14,text=fPurple] at (4.08,5.08) {LLM};
    \pic[scale=.72] at (3.50,4.55) {rh-summarize};
    \node[title] at (3.50,3.88) {4. Merge};
    \node[tiny] at (3.50,3.61) {across tasks};

    \draw[offlinecard,draw=fPurple,line width=.9pt] (4.75,3.42) rectangle (6.65,5.34);
    \node[badge,fill=fPurple!14,text=fPurple] at (6.28,5.08) {LLM};
    \pic[scale=.58] at (5.70,4.58) {rh-database};
    \node[title,text=fPurple] at (5.70,3.88) {5. Update};
    \node[tiny] at (5.70,3.61) {Meta-Skill $\mathcal{M}$};

    \draw[flow,draw=fPurple!70] (2.25,4.38) -- (2.55,4.38);
    \draw[flow,draw=fPurple!70] (4.45,4.38) -- (4.75,4.38);

    % Reuse the learned skill on the next batch.
    \draw[interaction,draw=fPurple] (5.70,3.42) -- (5.70,2.96)
      -- (.18,2.96) -- (.18,8.05) -- (.35,8.05);
    \node[tiny,text=fPurple,fill=fPurplePale,inner sep=1pt]
      at (3.15,2.96) {reuse $\mathcal{M}^{(r)}$ for the next batch};

    % ==================================================================
    % Online
    % ==================================================================
    \fill[draw=fBlue!35,fill=fBluePale,rounded corners=7pt,line width=.75pt]
      (7.30,1.45) rectangle (15.35,9.58);
    \node[heading,anchor=west,text=fBlue] at (7.60,9.22)
      {ONLINE: evolve one active run};
    \node[badge,fill=fBlue!12,text=fBlue] at (14.55,9.22)
      {$\mathcal{M}$ FROZEN};

    % Frozen Meta-Skill guidance spans all checkpoint calls.
    \draw[deploy] (6.65,4.38) -- (7.12,4.38) -- (7.12,8.30) -- (7.62,8.30);
    \node[tiny,text=fPurple,fill=white,inner sep=1pt,rotate=90]
      at (7.12,6.30) {deploy};
    \draw[onlinecard,draw=fPurple!65] (7.62,8.02) rectangle (14.95,8.62);
    \pic[scale=.27] at (8.08,8.32) {rh-database};
    \node[title,text=fPurple] at (11.28,8.32) {Frozen Meta-Skill guidance};

    \node[badge,fill=fPurple!14,text=fPurple] at (8.10,7.62) {LLM};
    \node[small,anchor=west,text=fPurple] at (8.48,7.62)
      {Evolver calls at checkpoints};

    % Repeated evolver calls, without repeated decision boxes.
    \foreach \x in {8.45,10.95,13.55} {
      \pic[scale=.62] at (\x,6.86) {rh-agent};
      \node[tiny,text=fPurple] at (\x,6.42) {Evolver};
      \draw[interaction,draw=fPurple] (\x,8.02) -- (\x,7.25);
    }

    \node[small] at (8.45,6.05) {$x+\Delta\tau^{(1)}$};

    \node[small] at (10.95,6.05) {$\Delta\tau^{(k)}+\sigma^{(k-1)}$};

    \pic[scale=.28] at (12.85,6.06) {rh-rubric};
    \node[small] at (13.70,6.05) {$\Delta\tau^{(K)}+$ state};
    \node[badge,fill=fTeal!14,text=fTeal] at (13.55,5.70) {ACCEPT / BACK};

    % Same task agent continues along one timeline.
    \draw[onlinecard,draw=fBlue!70,fill=white]
      (7.62,2.45) rectangle (14.95,4.70);
    \node[title,anchor=west] at (7.88,4.38) {Task Agent};
    \node[badge,fill=fPurple!14,text=fPurple] at (10.05,4.38) {LLM};
    \node[small,anchor=west,text=fGray] at (7.88,4.02)
      {one environment; one continuous trajectory};

    \pic[scale=.50] at (8.00,3.28) {rh-agent};
    \draw[draw=fBlue,line width=1.15pt] (8.42,3.02) -- (14.55,3.02);
    \foreach \x in {8.45,10.95,13.55}
      \fill[white,draw=fBlue,line width=1pt] (\x,3.02) circle (.11);
    \node[tiny,text=fBlue] at (8.45,2.72) {$t_1$};
    \node[tiny,text=fBlue] at (10.95,2.72) {$t_k$};
    \node[tiny,text=fBlue] at (13.55,2.72) {$t_K=T$};
    \node[tiny,text=fTeal] at (14.55,2.72) {artifact};

    \draw[interaction] (8.45,5.48) -- (8.45,3.13);
    \draw[interaction] (10.95,5.48) -- (10.95,3.13);
    \draw[interaction] (13.55,5.48) -- (13.55,3.13);

    \pic[scale=.38] at (8.10,5.12) {rh-settings};
    \node[tiny,anchor=west,text=fBlue,fill=fBluePale,inner sep=1pt]
      at (8.42,5.12) {Keep or evolve via notice $\cdot$ prompt $\cdot$ hook $\cdot$ tool};
    \node[badge,fill=fBlue!12,text=fBlue] at (13.65,4.78)
      {MECHANICAL CHECKPOINTS};

    % ==================================================================
    % Compact legend
    % ==================================================================
    \fill[draw=fGray!30,fill=fGrayPale,rounded corners=5pt,line width=.6pt]
      (0,.05) rectangle (15.35,1.08);
    \node[badge,fill=fPurple!14,text=fPurple] at (.72,.56) {LLM};
    \node[small,anchor=west] at (1.12,.56) {model call};
    \node[badge,fill=fBlue!12,text=fBlue] at (3.55,.56) {MECHANICAL};
    \node[small,anchor=west] at (4.30,.56) {routing / pairing};
    \node[badge,fill=fOrange!16,text=fOrange] at (7.25,.56) {VERIFIER};
    \node[small,anchor=west] at (7.85,.56) {offline only};
    \node[small,text=fGray] at (12.70,.56)
      {Online: $\mathcal{M}$ frozen; no verifier};

    \end{tikzpicture}%
    }
    \endgroup
    \caption{\textbf{Implementation flow for offline Meta-Skill learning and
    online harness evolution.} Offline, LLM agents collect A/B/C rollouts and
    deterministic outcome pairing creates \texttt{act}, \texttt{avoid}, and
    \texttt{hold} contrasts. LLM calls then write contrast-grounded lessons,
    merge recurring lessons across tasks, and update the Meta-Skill. Online,
    the frozen Meta-Skill guides an evolver LLM at deterministic checkpoints
    while the same task-agent LLM continues in one environment. The verifier
    is unavailable online.}
    \label{fig:experience-construction}
\end{figure}

==> figures/f3_payoff.tex <==
% Draft empirical layout. Intentionally contains no observations, curves,
% numerical ticks, or uncertainty intervals. Populate only from matched runs.
\begin{figure}[t]
    \centering
    \begingroup
    \definecolor{rpInk}{HTML}{283B50}
    \definecolor{rpBlue}{HTML}{376FA6}
    \definecolor{rpOrange}{HTML}{B65B27}
    \definecolor{rpTeal}{HTML}{287F83}
    \definecolor{rpPale}{HTML}{F5F7FA}
    \begin{tikzpicture}[
        x=.91cm,y=.90cm,
        font=\sffamily\fontsize{8}{9.5}\selectfont,text=rpInk,
        axis/.style={draw=rpInk!70,line width=.6pt},
        title/.style={font=\sffamily\bfseries\fontsize{8.5}{10}\selectfont},
        note/.style={font=\sffamily\fontsize{7}{8.5}\selectfont,align=center},
        pending/.style={font=\sffamily\bfseries\fontsize{9}{11}\selectfont,
                        text=rpInk!50,align=center},
        panel/.style={draw=rpInk!12,fill=white,rounded corners=4pt,line width=.5pt}
    ]
    % Status is embedded in the artwork, not only in the caption.
    \fill[rounded corners=4pt,rpPale] (0,6.43) rectangle (15.2,7.02);
    \node[title] at (7.60,6.73) {DRAFT LAYOUT --- MATCHED RESULTS PENDING};
    \draw[panel] (0,1.44) rectangle (4.83,6.22);
    \draw[panel] (5.18,1.44) rectangle (10.01,6.22);
    \draw[panel] (10.37,1.44) rectangle (15.20,6.22);
    \node[title] at (2.415,5.89) {A. Online efficiency};
    \node[title] at (7.595,5.89) {B. Rescue and harm};
    \node[title] at (12.785,5.89) {C. Payoff from reuse};

    % A: future observations across predeclared matched budget settings.
    \draw[axis] (.89,5.38) -- (.89,3.00) -- (4.49,3.00);
    \node[note,rotate=90] at (.34,4.20) {Task success (\%)};
    \node[note] at (2.69,2.65) {Total online tokens / task};
    \node[pending] at (2.69,4.25) {PENDING};
    \node[note,text=rpInk!55] at (2.69,3.80) {No measurements plotted};
    \node[note,text width=3.75cm] at (2.415,1.97)
      {Worker + supervisor tokens\\Matched tasks; budget sweep};

    % B: two conditional rates, not a net score or checkpoint causal estimate.
    \draw[axis] (6.07,5.38) -- (6.07,3.00) -- (9.67,3.00);
    \draw[axis] (6.93,3.00) -- (6.93,2.92);
    \draw[axis] (8.87,3.00) -- (8.87,2.92);
    \node[note,rotate=90] at (5.52,4.20) {Paired-run rate (\%)};
    \node[note] at (6.93,2.65) {Rescue};
    \node[note] at (8.87,2.65) {Harm};
    \node[pending] at (7.87,4.25) {PENDING};
    \node[note,text=rpInk!55] at (7.87,3.80) {With / without Meta-Skill};
    \node[note,text width=3.75cm] at (7.595,1.97)
      {Rescue: reference failures\\Harm: reference successes};

    % C: no illustrative declining curve or unmeasured break-even point.
    \draw[axis] (11.26,5.38) -- (11.26,3.00) -- (14.86,3.00);
    \node[note,rotate=90] at (10.71,4.20) {Cost / task (USD)};
    \node[note] at (13.06,2.65) {Number of deployments $N$};
    \node[pending] at (13.06,4.25) {PENDING};
    \node[note,text=rpInk!55] at (13.06,3.80) {Matched cost accounting};
    \node[note,text width=3.75cm] at (12.785,1.97)
      {Offline cost / $N$ + mean online cost\\Compare at similar task success};

    % Planned series are illustrated only in this legend, outside plot areas.
    \node[note,anchor=west,text=rpInk!65] at (.18,1.13)
      {Planned comparisons (A, C: all four; B: the two online-supervision variants)};
    \fill[rpInk!65] (.49,.69) circle (.06);
    \node[note,anchor=west] at (.73,.69) {Worker only};
    \fill[rpBlue] (7.67,.62) rectangle (7.81,.76);
    \node[note,anchor=west] at (7.98,.69) {Pre-task customization};
    \fill[rpOrange] (.49,.33) -- (.39,.16) -- (.59,.16) -- cycle;
    \node[note,anchor=west] at (.73,.24) {Online supervision without Meta-Skill};
    \fill[rpTeal] (7.74,.34) -- (7.84,.24) -- (7.74,.14) -- (7.64,.24) -- cycle;
    \node[note,anchor=west] at (7.98,.24) {\method (full)};
    \end{tikzpicture}
    \endgroup
    \caption{\textbf{Does rehearsing offline pay off online? Planned empirical
    figure; every panel is pending.}
    (A) Success versus actual online token use across matched budget settings.
    (B) Rescue and harm for supervision with and without Meta-Skill, each paired
    with the same worker-only reference; denominators are reference failures
    and successes, respectively. Planned intervals use task-clustered resampling;
    zero denominators are not estimable. (C) Amortized offline-plus-online cost
    under Equation~\ref{eq:amortized-cost}, assessed alongside task success.
    Setup costs are included where applicable. Axes specify intended readouts,
    not observed trends; no points, bars, curves, or error intervals are plotted.
    The earlier-pipeline scores are not substituted for these matched runs.}
    \label{fig:precompute-payoff}
\end{figure}

==> figures/rehearse_icons.tex <==
% Original, editable vector symbols for the REHEARSE overview.
% All colors and line styles are inherited from the enclosing figure.
\tikzset{
  pics/rh-workflow/.style={code={
    \draw[icon,draw=rhBlue] (-.31,.22) -- (.31,.22) -- (0,-.25) -- cycle;
    \foreach \x/\y in {-.31/.22,.31/.22,0/-.25}
      \draw[icon,fill=rhBluePale] (\x,\y) circle (.105);
  }},
  pics/rh-supervisor/.style={code={
    % A centered monitoring eye: one silhouette, no overlapping accessories.
    \draw[icon,fill=white,rounded corners=2pt]
      (-.50,-.25) rectangle (.50,.39);
    \draw[icon,draw=rhTeal,fill=rhTealPale]
      (-.34,.07) .. controls (-.16,.32) and (.16,.32) .. (.34,.07)
      .. controls (.16,-.18) and (-.16,-.18) .. cycle;
    \fill[rhTeal] (0,.07) circle (.105);
    \draw[icon] (0,-.25) -- (0,-.43);
    \draw[icon] (-.22,-.43) -- (.22,-.43);
  }},
  pics/rh-agent/.style={code={
    \draw[icon,fill=white,rounded corners=3pt] (-.43,-.26) rectangle (.43,.28);
    \draw[icon] (0,.28) -- (0,.47);
    \fill[rhBlue] (0,.49) circle (.055);
    \fill[rhBlue] (-.18,.04) circle (.063);
    \fill[rhBlue] (.18,.04) circle (.063);
    \draw[icon,draw=rhBlue] (-.13,-.13) -- (.13,-.13);
    \draw[icon,fill=rhBluePale,rounded corners=1pt]
      (-.53,-.12) rectangle (-.43,.14);
    \draw[icon,fill=rhBluePale,rounded corners=1pt]
      (.43,-.12) rectangle (.53,.14);
  }},
  pics/rh-terminal/.style={code={
    \draw[icon,fill=white,rounded corners=2pt] (-.50,-.30) rectangle (.50,.34);
    \draw[icon] (-.50,.17) -- (.50,.17);
    \foreach \x in {-.38,-.27,-.16} \fill[rhOrange] (\x,.255) circle (.024);
    \draw[icon,draw=rhOrange] (-.31,.04) -- (-.21,-.035) -- (-.31,-.11);
    \draw[icon,draw=rhOrange] (-.09,-.11) -- (.21,-.11);
    \draw[icon] (-.12,-.30) -- (-.12,-.43) -- (.12,-.43) -- (.12,-.30);
    \draw[icon] (-.29,-.43) -- (.29,-.43);
  }},
  pics/rh-document/.style={code={
    \draw[icon,fill=white] (-.29,-.39) -- (.29,-.39) -- (.29,.22)
      -- (.12,.39) -- (-.29,.39) -- cycle;
    \draw[icon] (.12,.39) -- (.12,.22) -- (.29,.22);
    \foreach \y in {.13,-.01,-.15} \draw[icon,draw=rhBlue!65] (-.18,\y) -- (.15,\y);
  }},
  pics/rh-distill/.style={code={
    % A funnel extracts a compact lesson from many observations.
    \foreach \x/\y in {-.28/.43,0/.53,.28/.43}
      \fill[rhBlue] (\x,\y) circle (.055);
    \draw[icon,fill=rhBluePale] (-.47,.25) -- (.47,.25)
      -- (.12,-.12) -- (.12,-.33) -- (-.12,-.44)
      -- (-.12,-.12) -- cycle;
    \fill[rhTeal] (0,-.55) circle (.065);
  }},
  pics/rh-summarize/.style={code={
    % Multiple lessons converge into one synthesized reference.
    \foreach \x in {-.36,0,.36} {
      \draw[icon,draw=rhBlue] (\x,.24) -- (0,-.02);
      \draw[icon,fill=white,rounded corners=1pt]
        (\x-.10,.24) rectangle (\x+.10,.49);
    }
    \draw[icon,draw=rhTeal] (0,-.02) -- (0,-.15);
    \draw[icon,draw=rhTeal,fill=rhTealPale,rounded corners=2pt]
      (-.32,-.54) rectangle (.32,-.15);
    \draw[icon,draw=rhTeal] (-.20,-.28) -- (.20,-.28)
      (-.20,-.41) -- (.12,-.41);
  }},
  pics/rh-database/.style={code={
    \path[fill=rhTealPale] (-.62,.36) -- (-.62,-.33)
      arc[start angle=180,end angle=360,x radius=.62,y radius=.18]
      -- (.62,.36) -- cycle;
    \draw[icon,draw=rhTeal] (-.62,.36) -- (-.62,-.33)
      arc[start angle=180,end angle=360,x radius=.62,y radius=.18] -- (.62,.36);
    \draw[icon,draw=rhTeal] (-.62,.02)
      arc[start angle=180,end angle=360,x radius=.62,y radius=.18];
    \draw[icon,draw=rhTeal] (-.62,-.16)
      arc[start angle=180,end angle=360,x radius=.62,y radius=.18];
    \draw[icon,fill=white,draw=rhTeal] (0,.36) ellipse[x radius=.62,y radius=.18];
  }},
  pics/rh-profile/.style={code={
    \fill[rhBlue!45,rounded corners=1pt] (-.35,-.26) rectangle (-.19,.05);
    \fill[rhBlue!70,rounded corners=1pt] (-.07,-.26) rectangle (.09,.32);
    \fill[rhBlue,rounded corners=1pt] (.21,-.26) rectangle (.37,.17);
    \draw[icon] (-.43,-.30) -- (.44,-.30);
  }},
  pics/rh-rubric/.style={code={
    \draw[icon,fill=white,rounded corners=1pt] (-.31,-.36) rectangle (.31,.33);
    \draw[icon,fill=rhBluePale,rounded corners=1pt] (-.13,.24) rectangle (.13,.40);
    \foreach \y in {.12,-.05,-.22} {
      \draw[icon,draw=rhTeal] (-.22,\y) -- (-.17,\y-.05) -- (-.09,\y+.05);
      \draw[icon,draw=rhBlue!65] (.00,\y) -- (.21,\y);
    }
  }},
  pics/rh-speech/.style={code={
    \draw[icon,fill=white,rounded corners=2pt]
      (-.43,-.14) -- (-.43,.31) -- (.43,.31) -- (.43,-.14)
      -- (-.10,-.14) -- (-.30,-.33) -- (-.30,-.14) -- cycle;
    \foreach \x in {-.21,0,.21} \fill[rhOrange] (\x,.085) circle (.04);
  }},
  pics/rh-settings/.style={code={
    \draw[icon,fill=white,rounded corners=2pt] (-.42,-.35) rectangle (.42,.35);
    \foreach \y/\x in {.20/-.12,0/.16,-.20/-.04} {
      \draw[icon,draw=rhOrange] (-.28,\y) -- (.28,\y);
      \draw[icon,draw=rhOrange,fill=white] (\x,\y) circle (.057);
    }
  }},
  pics/rh-pass/.style={code={
    \fill[rhTealPale] (0,0) circle (.15);
    \draw[draw=rhTeal,line width=1pt,line cap=round,line join=round]
      (-.085,0) -- (-.02,-.07) -- (.10,.075);
  }},
  pics/rh-fail/.style={code={
    \fill[rhOrangePale] (0,0) circle (.15);
    \draw[draw=rhOrange,line width=1pt,line cap=round]
      (-.07,-.07) -- (.07,.07) (-.07,.07) -- (.07,-.07);
  }}
}

==> include/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> tables/ablation_study.tex <==
\begin{table}[H]
    \centering
    \caption{\textbf{Component ablation.} Cumulative results on
    Terminal-Bench 2.1 and DeepSWE 1.1.}
    \label{tab:component-ablations}
    \vspace{4pt}
    \definecolor{ablationlightbrown}{rgb}{0.99,0.96,0.93}
    {%
    \renewcommand{\arraystretch}{1.12}
    \setlength{\tabcolsep}{9pt}
    \small
    \begin{tabular}{lcc}
        \toprule[1.5pt]
        \textbf{Configuration} & \textbf{Terminal-Bench 2.1} &
        \textbf{DeepSWE 1.1} \\
        \midrule[1.2pt]
        Task agent & 66.33 & 34.67 \\
        + Evolver & 74.67 & 36.44 \\
        + Meta-Skill (self-distilled) & 77.00 & 35.56 \\
        \rowcolor{ablationlightbrown}
        \textbf{+ Meta-Skill (contrastive; Full)} &
        \textbf{81.00} & \textbf{44.44} \\
        \bottomrule[1.5pt]
    \end{tabular}
    }
\end{table}
